Superpixels algorithms through network community detection

Community detection is a powerful tool from complex networks analysis that finds applications in various research areas. Several image segmentation methods rely for instance on community detection algorithms as a black box in order to compute undersegmentations, i.e. a small number of regions that represent areas of interest of the image. However, to the best of our knowledge, the efficiency of such an approach w.r.t. superpixels, that aim at representing the image at a smaller level while preserving as much as possible original information, has been neglected so far. The only related work seems to be the one by Liu et. al. (IET Image Processing, 2022) that developed a superpixels algorithm using a so-called modularity maximization approach, leading to relevant results. We follow this line of research by studying the efficiency of superpixels computed by state-of-the-art community detection algorithms on a 4-connected pixel graph, so-called pixel-grid. We first detect communities on such a graph and then apply a simple merging procedure that allows to obtain the desired number of superpixels. As we shall see, such methods result in the computation of relevant superpixels as emphasized by both qualitative and quantitative experiments, according to different widely-used metrics based on ground-truth comparison or on superpixels only. We observe that the choice of the community detection algorithm has a great impact on the number of communities and hence on the merging procedure. Similarly, small variations on the pixel-grid may provide different results from both qualitative and quantitative viewpoints. For the sake of completeness, we compare our results with those of several state-of-the-art superpixels algorithms as computed by Stutz et al. (Computer Vision and Image Understanding, 2018).

==> plots/communities/legends.tex <==
{\scriptsize
    \begin{tabularx}{0.6\textwidth}{X X l}
        \ref{plot:lvn} \LVN &
        \ref{plot:lp} \LPB \\ 
        \ref{plot:inf} \INF &
    \end{tabularx}
}


==> plots/legends.tex <==
{\scriptsize
    \begin{tabularx}{0.675\textwidth}{X X X l}
        \ref{plot:inf} \INF &
        \ref{plot:eams} \EAMS &
        \ref{plot:ers} \ERS \\
        \ref{plot:fh} \FH &
        \ref{plot:qs} \QS &
        \ref{plot:slic} \SLIC \\
        \ref{plot:seeds} \SEEDS &
        \ref{plot:tps} \TPS &
        \ref{plot:etps} \ETPS &
    \end{tabularx}
}


==> plots/references.tex <==
\begin{tikzpicture}
    \begin{axis}[hide axis]
        \addplot [LVN,forget plot] coordinates{(1,1)};\label{plot:lvn} % 1
        \addplot [LP,forget plot] coordinates{(1,1)};\label{plot:lp} % 1
        \addplot [INF,forget plot] coordinates{(1,1)};\label{plot:inf} % 1
        \addplot [EAMS,forget plot] coordinates{(1,1)};\label{plot:eams} % 2
        \addplot [FH,forget plot] coordinates{(1,1)};\label{plot:fh} % 4
        \addplot [QS,forget plot] coordinates{(1,1)};\label{plot:qs} % 7
        \addplot [SLIC,forget plot] coordinates{(1,1)};\label{plot:slic} % 12
        \addplot [SEEDS,forget plot] coordinates{(1,1)};\label{plot:seeds} % 17
        \addplot [TPS,forget plot] coordinates{(1,1)};\label{plot:tps} % 20
        \addplot [ERS,forget plot] coordinates{(1,1)};\label{plot:ers} % 30
        \addplot [ETPS,forget plot] coordinates{(1,1)};\label{plot:etps} % 30
    \end{axis}
\end{tikzpicture}

